A rigorous formulation of and partial results on Lorenz's "consensus strikes back" phenomenon for the Hegselmann-Krause model

In a 2006 paper, Jan Lorenz observed a curious behaviour in numerical simulations of the Hegselmann-Krause model: Under some circumstances, making agents more closed-minded can produce a consensus from a dense configuration of opinions which otherwise leads to fragmentation. Suppose one considers initial opinions equally spaced on an interval of length $L$. As first observed by Lorenz, simulations suggest that there are three intervals $[0, L_1)$, $(L_1, L_2)$ and $(L_2, L_3)$, with $L_1 \approx 5.23$, $L_2 \approx 5.67$ and $L_3 \approx 6.84$ such that, when the number of agents is sufficiently large, consensus occurs in the first and third intervals, whereas for the second interval the system fragments into three clusters. In this paper, we prove consensus for $L \leq 5.2$ and for $L$ sufficiently close to 6. These proofs include large computations and in principle the set of $L$ for which consensus can be proven using our approach may be extended with the use of more computing power. We also prove that the set of $L$ for which consensus occurs is open. Moreover, we prove that, when consensus is assured for the equally spaced systems, this in turn implies asymptotic almost sure consensus for the same values of $L$ when initial opinions are drawn independently and uniformly at random. We thus conjecture a pair of phase transitions, making precise the formulation of Lorenz's "consensus strikes back" hypothesis. Our approach makes use of the continuous agent model introduced by Blondel, Hendrickx and Tsitsiklis. Indeed, one contribution of the paper is to provide a presentation of the relationships between the three different models with equally spaced, uniformly random and continuous agents, respectively, which is more rigorous than what can be found in the existing literature.

==> uniform.tex <==
\newcommand{\diam}[2]{\text{span}_{#1}(#2)} 

In this section we will prove the first half of Theorem \ref{thm:intro1}, that $C_\text{Eq}(L) = 1$ for any $L \in [0,\, 5)$.


  Our stategy will be to first, for some fixed $n$ and some set of diameters $L_j$, explicitly compute the fifth update $U^5 f^{n,L_j}$ of the corresponding canonical equidistant profiles. For each diameter, we will use the theory developed in the last section to bound the opinions of the extremists of $(f^{n,L_j})^{(k)}$ and thus show that the diameter of any such refinement is below 2. The continuity established in Lemma \ref{lem:cont} will then give us bound the diameter of the fifth update of the canonical linear profile as $D(U^5 f^{L_j}) < 2$, which in turn implies the frozen profile must be a consensus by the last part of Corollary \ref{cor:regularity}. We will set some common initial left and right deviation bounds $e_l^0$ and $e_r^0$ and choose the values $L_j$ densely enough on $[0,\,5)$ so that for \emph{any} $L$ in the interval $e_l^0$ and $e_r^0$ will bound the deviation $(f^{n,L} - f^{n,L_j})$ for some $j$.



% we will use the theory developed in the previous section to cast new light on the the mysteries of uniformly generated opinions under the Hegselmann-Krause dynamics, which is probably the most studied case.
% 
% On the one hand, when $n$ opinions are chosen independently and uniformly at random from an interval of length $L$, simulations tend to show that the resulting behaviour is somewhat chaotic: Even for fairly large choices of $n$, say $10^5$ or $10^6$, the final distribution of the agents may vary substantially between runs of the simulation.
% 
% On the other hand, as $n$ is made sufficiently large, patterns start to emerge. If $L$ is small enough, any large enough $n$ will produce a profile that eventually reaches a consensus. For $L \leq 3$ a hundred agents are enough that in practice every run reach a consensus, and for $L \leq 4$ a thousand agents are nearly always enough. If we increase $L$ further, we see that somewhere slightly above $L=5$ profiles start to fragment into clusters, and the larger we choose $L$ the more clusters we tend to get. This pattern is simple and holds for $n$ up to at least a few hundred thousand, and so it is tempting to believe that it will hold as $n$ grows arbitrarily large, and thus also hold for linear continuous profiles.
% 
% It seems, however, that this intuition is only partially right, and we will devote this section to scrutinising the behaviour of linear profiles, using the hitherto developed theory. For a positive real number $L$, let $g_L$ denote the profile for which $g_L(\alpha) = L \alpha$,\sout{and let $K(L)$ be the number of clusters in $U^\infty g_L$. It appears as though $K$ is not monotone in $L$, but instead increases and decreases in a complicated although somewhat regular manner.}

% 
% To the best of our currant understanding, the $K$ seems to be constant outside a set of breaking points, and the approximate behaviour is given in the following table.
% 
% \begin{center}
% % \begin{tabular}{r | l}
% % %  \toprule
% %   $L$ & $K(L)$ \\%&  of clusters (including nanoclusters) \\
% %   \midrule
% %   \begin{tabular}{@{}c@{}}
% %     0 \\    % \hline
% %     5.23 \\ % \hline
% %     5.67 \\ % \hline
% %     6.84 \\ % \hline
% %     7.10 \\ % \hline
% %     9.84 \\ % \hline
% %     10.22\\ % \hline
% %     11.60\\ % \hline
% %     11.65\\ % \hline
% %     14.33\\ % \hline
% %     14.70
% %   \end{tabular} &
% %   \begin{tabular}{@{}c@{}}
% %     1\\ 
% %     3\\ 
% %     1\\ 
% %     3\\ 
% %     5\\ 
% %     7\\ 
% %     5\\ 
% %     7\\ 
% %     9\\ 
% %     11\\
% %   \end{tabular}
% %   % & 
% %   % \begin{tabular}{@{}c@{}}
% %   %   \\
% %   %   \\
% %   %   \\
% %   %   \\
% %   %   \\
% %   %   \\
% %   %   \\
% %   %   \\
% %   %   \\
% %   % \end{tabular} 
% % \end{tabular}
% 
%   \begin{tabular}{c c}
%     $L$ & $K(L)$ \\%&  of clusters (including nanoclusters) \\
%   \midrule
%     0     -- 5.23  & 1\\
%     5.23  -- 5.67  & 3\\ 
%     5.67  -- 6.84  & 1\\ 
%     6.84  -- 7.10  & 3\\ 
%     7.10  -- 9.84  & 5\\ 
%     9.84  -- 10.22 & 7\\ 
%     10.22 -- 11.60 & 5\\ 
%     11.60 -- 11.65 & 7\\ 
%     11.65 -- 14.33 & 9\\ 
%     14.33 -- 14.70 & 11  
%   \end{tabular}
% 
% 
% \end{center}
% 
% [[Den här tabellen är farlig! Förklarar jag varför den ser ut som den gör måste jag förklara varför 2r-förmodan är fel, vilket den är.]]
% 
% This table was created by observing the evolution of a large number of \emph{equidistant profiles}, a concept to be defined and thoroughly investigated below.
% 
% Despite considerable effort, we have not managed to show for certain that $K(L) > 1$ for any choice of $L$, but we conjecture that the table is accurate based of extensive simulations and heuristical arguments. \footnote{The number of agents used in our simulations exceed any that we have observed in other literature.} Below, we prove that a consensus is reached for some select values of $L$ in the first and third of the intervals in the table above.

Fix $\varepsilon>0$ and an odd number $n \geq 3$. Let $\left( f^{n,L_j} \right)_{j=1}^r$ denote a finite family of equidistant profiles, all with $n$ agents and increasing diameters $L_j$ chosen such that $L_{j+1} - L_j \leq 2\varepsilon$ for any $j \in [r-1]$. For each such $f^{n,L_i}$, define the following left and right deviation bounds:
\begin{align*}
  e_{r,j}(i) = 
  e_r(i) &= 
  \begin{cases}
    %\fnac{i - \frac{n+1}{2}}{\frac{n+1}{2}} & \text{if } i \geq \frac{n-1}{2} \\
    \frac{2i - n - 1}{n+1}\varepsilon & \text{if } i \geq \frac{n+1}{2} \\
    0  & \text{otherwise,}
  \end{cases}\\
  e_{l,j}(i) =
  e_{l}(i) &=
  \begin{cases}
    % \frac{i - \frac{r+1}{2}}{\frac{r-1}{2}} & \text{if } i \geq \frac{i-1}{2} \\
    \frac{n + 1 - 2i}{n+1}\varepsilon & \text{if } i \leq \frac{n+1}{2} \\
    0  & \text{otherwise.}
  \end{cases}
\end{align*}
Note that $e_r (\frac{n+1}{2}) = e_l (\frac{n+1}{2}) = 0$ and $e_l(1) = e_r(n) = \varepsilon$. These bounds are chosen so that, if every profile $f^{n,L_j}$ is shifted to the interval $[\frac{L_j}{2},\, \frac{L_j}{2}]$, each profile $f^{n,L_j}$ can be transformed into the profile $f^{n,L_{j+1}}$ by adding a deviation within these bounds.

\begin{theorem}
  Assume there is a time $T>0$ and a $\delta > 0$, such that the following hold for each $j \in [r-1]$.
  \begin{enumerate}
  \item $D(U^{t_j} f^{n,L_j}) \leq 2-2\delta$ for some $t_j \leq T$.
  \item Using the same notation as in Corollary \ref{cor:devprop}, we have $e_{r,j}^{t_j}(n) < \delta$ and  $e_{l,j}^{t_j}(1) < \delta$.
  \end{enumerate}
  Then, $U^\infty f_L$ is a consensus for every $L \in [L_1,\, L_r]$, where $f_L$ denotes the linear profile with diameter $L$.
\end{theorem}

\begin{corollary}
  $U^\infty f_{m,L}$ is a consensus for large enough $m$ for any $L \in [L_1,\, L_r]$.

  With $f^{m,L}$ denoting the profile with opinions chosen independently and uniformly at random from an interval of length $L$, $U^\infty f^{m,L}$ is a consensus a.a.s. for large $m$ for every $L [L_1,\, L_r]$.
\end{corollary}



--------------------------

In this section, we will investigate what happens when opinions are evenly spread on an interval. More precisely, we will consider updates of discrete profiles where all the distances between consecutive agents are the same, and compare them to those of their canonical regular refinements. We will find explicit formulae up to the second updates, and use these together with Corollary \ref{cor:devprop} to bound the differences in further updates. We will then use these bounds to prove Theorem \ref{thm:intro1}, and to obtain the partial results about the case where $L = 5.5$ which were promised in the introduction.


\begin{obs}\label{obs:transinv2}
  Define the BHT-regular profile $f_L$ by $f_L(\alpha) = L \alpha$. Then, a discrete profile $f$ is equidistant if and only if there exist numbers $n \in \mathbb{Z}_+$ and $L,\, C \in \mathbb{R}$ such that $f = B_k^n(f_L) + C$. Due to Observation \ref{obs:transinv}, we will henceforth assume $C=0$
\end{obs}

\begin{obs}
  An equidistant profile is symmetric, and will remain symmetric around its centre after any number of updates.
\end{obs}

%%%%%%-- Följande skulle kunna bli intressant:

% \begin{obs}\label{obs:continuity}
%   The linear continuous agent profile, which our equidistant profiles approximate, is regular. This implies that if we fix a diameter $L$ and a number $T$ of updates and let the number $n$ of agents go to infinity, the set of opinions after $T$ updates becomes dense, provided that the distance between the opposite extremists remains larger than $2$ after $T-1$ updates.
% \end{obs}
% 
% In other words, if we fix a diameter $L$ and consider the the $T$'th update of an equidistant profile on $[0,\, L]$, there are two possible results. Either
% \begin{enumerate}
% \item any open interval of opinions between the extremist opinions will contain an opinion held by some agent, provided that $n$ is large enough, or
% \item the diameter of the profile has shrunk to less than $2$ \emph{before} the $T$'th update.
% \end{enumerate}

For the rest of the section we will, for a given profile discrete $f$ with $n$ agents and a time $t \geq 0$, let $L_t$ denote the \emph{diameter at time $t$}, meaning that $L_t := U^tf(n) - U^tf(1)$.

% \begin{theorem}
%   Distribute $n$ agents equidistantly on the interval $[0,\, L]$. If, after some fixed number of updates, no two opinions in the profile differ by more than $2$, then the profile will eventually reach consensus, if $n$ is large enough.
% \end{theorem}
\begin{lemma}\label{thm:below2}
  Fix $L>0$, $t \in \mathbb{N}$, let $n \geq 3$ be an odd number, and let $f = B_\infty^n(f_L)$ be an equidistant profile with $n$ agents and diameter $L$. Then the following closely related statements hold.
  \begin{enumerate}[label = {\alph*)}]
  \item If the diameter of $U^t f$ is less than 2, then $U^\infty f$ is a consensus.\label{lem:below2a}

  \item Further, fix some left and right bounds $e_l^0$ and $e_r^0$, and compute $e_l^t$ and $e_r^t$ from $f$, $e_l^0$ and $e_r^0$ using Corollary \ref{cor:devprop}. 
    Now, if the diameter of $U^t f$ is smaller than or equal to
    \begin{align*}
      2 - e_l^t(1) - e_r^t(n)
    \end{align*}
    then $U^\infty f^{(k)}$ is a consensus for every $k \in \mathbb{N}$.\label{lem:below2b}

  \item Under the assumptions of \ref{lem:below2b}, $U^\infty f_L$ is a consensus.\label{lem:below2c}

%   \item Let $g$ be a profile with $n_r$ agents, with opinions drawn independently and uniformly at random from an interval of length $L$. Then $U^\infty g$ is asymptotically almost surely a consensus as $n_r \to \infty$, i.e. $C_{rand}(L) = 1$.
%     \label{lem:below2d}
    
  \end{enumerate}

\end{lemma}



\begin{taggedblock}{proofsuniform}
\begin{proof}
  %First, assume $n$ is odd. Then
  For \ref{lem:below2a} and \ref{lem:below2b}, as $n$ is odd, there will be an agent that initially holds the opinion $\frac{L}{2}$, and, by symmetry, will retain this opinion until the system freezes. In the case of \ref{lem:below2a}, as the distance between the extremists are certainly less than $2$, they both must be within distance $1$ from the central opinion, again by symmetry. This will cause the extremists to move towards the centre until a consensus is reached. This proves \ref{lem:below2a}.

  To prove \ref{lem:below2b}, we know that the extremists must be within sight of the centre, regardless the choice of $k$. With at least one agent in the centre, the extremist opinions will change by at least $\frac{2}{n + (n-1)k - 1}$ at every update, and must thus eventually see each other and reach consensus. This proves \ref{lem:below2b}.

  As for \ref{lem:below2c}, note that $f_L = U^0 f_L$ is regular for any $L$. From the previous parts and Lemma \ref{lem:cont}, by Lemma \ref{lem:regularity}, there must thus be some last time $t_0 \leq t$ for which $U^{t_0}g_l$ is regular with diameter ${2 - 2\delta}$ for some $\delta > 0$. If $M$ is the upper bound for the derivative of $U^{t_0}g_l$, it follows that the measure of the set of agents who can see both extremists must be at least $\frac{2 \delta}{M}$. These agents will thus form a cluster in the centre of $U^{t_0 + 1}g_l$ which cannot be broken up or change it's opinion, yet again by symmetry. By the same argument as above, this implies that the profile must eventually reach a consensus. This proves \ref{lem:below2c}.

%   For \ref{lem:below2d}, choose $t_0$ and $\delta$ as above and note that with by Corollary \ref{cor:glivcan} and Observation \ref{obs:regular}, if $n_r$ is large enough,
%   \begin{align}\label{eq:below2d}
%     ||U^{t_0} g - U^{t_0} f_L||_\infty < \frac{\delta}{4}
%   \end{align}
%   with high probability. Assuming this is holds, we get that
%   \begin{align}
%     | \langle U^{t_0} g (i) \rangle_{i \in [n_r]} - \frac{L}{2}| < \frac{\delta}{4}
%   \end{align}
%   with high probability.  Using this and the same argument as above, we deduce that the measure of the set, call it $C$, of agents in $U^{t_0} g$ who can see every other agent is at least $\frac{\delta}{M}$. These agents must all hold the global average opinion of $U^{t_0} g$ in $U^{t_0 + 1} g$, which we have seen differs at most $\frac{\delta}{4}$ from $\frac{L}{2}$. 
%   By \eqref{eq:below2d} and the way $t_0$ was defined, we see that 
%   
%   ...
% 
%   ... 
  
  
  
  %If we want to avoid using the parity of $n$, we can instead use Observation \ref{obs:continuity}: Say that the diameter after of $U^T B_\infty^n$ is above two and that the diameter after $T+1$ updates is $2-2\varepsilon$ for some $\varepsilon>0$. Then the profile $U^{T+1} f_L$ will be regular by the observation, and thus there will be some agent with an opinion in the interval $[\frac{L}{2} -\varepsilon,\, \frac{L}{2} + \varepsilon]$. This agent now has every other agent as a neighbour, and will thus after the next update assume the average opinion of the profile, which by symmetry must be $\frac{L}{2}$. We may then proceed as in the case of an odd $n$.
\end{proof}
\end{taggedblock}


% \begin{comment}
% \begin{definition}
%   An agent whose opinion is affected by the $t$'th update, but not by the $(t-1)$'th is said to be of generation $t$.
% \end{definition}
% 
% \begin{rem}\label{rem:gen}
%   To find to which generation an agent in an equidistant profile belong, one may take the smallest initial distance to an extremist and round up to the nearest integer. This is obvious.(?)
% \end{rem}
% \end{comment}

\begin{corollary}\label{cor:cons1}
  Let $f$ be an equidistant profile  with $n$ agents and diameter $L$, and, for some $t_0\geq 0$, let $e_r^{t_0}$ and $e_l^{t_0}$ be left and right bounds on the deviation $e = B^{n}_{k} (U^{t_0} f^{(k)}) - U^{t_0} f$.
  %a consistent deviation $e$ of $U^{t_0}f$.

  If, with the notation from Corollary \ref{cor:devprop}, for some $t_1 \geq t_0$ we have that
  \begin{equation*}
    U^{t_1}f(n) - U^{t_1}f(1) + e_r^{t_1}(n) + e_l^{t_1}(1) < 2,
  \end{equation*}
  then, for any choice of an even natural number $2k$, $U^{t_2}f^{(2k)}$ is a consensus for some $t_2$.

%  Moreover, this implies that the random profile $g_m$ with $m$ agents where the opinions are drawn independently and uniformly at random from an interval of length $L$ will asymptotically almost surely reach a consensus as $m \to \infty$.
\end{corollary}
\begin{taggedblock}{proofsuniform}
\begin{proof}
%  For the first part,
  Simply note that Corollary \ref{cor:devprop} ensures us that the diameter of $U^{t_2}f^{(2k)}$ is smaller than $2$ and that symmetry is preserved. Then apply Lemma \ref{thm:below2}.
% 
%   For the second part, it follows by the Glivenco-Cantelli Lemma that
%   \begin{equation*}
%     \lim_{\substack{k \to \infty \\ m \to \infty}} ||f^{(2k)} - g_m||_\infty \to 0
%   \end{equation*}
%   almost surely. By the continuity established in Lemma \ref{lem:cont} this extends to
%   \begin{equation*}
%     \lim_{\substack{k \to \infty \\ m \to \infty}} ||U^{t_2}f^{(2k)} - U^{t_2}g_m||_\infty \to 0,
%   \end{equation*}
%   almost surely.
%   %As the diameter of $U^{t_2}f^{(2k)}$ is strictly less than $2$ for any $k$ by the first part, this implies that so is $U^{t_2}g_m$, a.a.s as $m \to \infty$.
%  As $U^{t_2} f^{(2k)}$ is a consensus, this implies that
%  \begin{equation}
%         U^{t_2}g_m (m) - U^{t_2}g_m (1) \leq 1
% \end{equation}
%   a.a.s as $m \to \infty$, and so $U^{t_2+1} g_m$ is a consensus a.a.s.
\end{proof}
\end{taggedblock}





\begin{corollary}
  %Let $g_n$ be a profile with $n$ agents drawn independently and uniformly at random from an interval of length $L=5$. Then $\lim_{T \to \infty} U^Tg_n$ is a consensus a.a.s. as $n \to \infty$
  Let $f$ be an equidistant profile with $n$ agents and diameter $L \leq 5.1$ (?). Then $\lim_{T \to \infty} \lim^{n \to \infty}  U^T f =\lim_{T \to \infty} U^T f_L $ is a consensus.
\end{corollary}

\begin{taggedblock}{proofsuniform}
  \begin{proof}
   
    
    Fix $n = 10000$ (?) and $\delta = 10^{-3}$(?), and define profiles $f_L = B_\infty^n(f_L)$. For each $L \in \{ 2,\, 2 + \delta,\, 2 + 2 \delta,\, ...,\, 5.1\}$, compute the 5th update $U^5 f_L$, along with the bounds $e_l^5$ and $e_r^5$ seeded with $e_l^0(i) = e_r^0(i) = \delta$ for all $i \in [n]$. Such calculations show that this will eventually result in a consensus by \ref{cor:cons1}.

    Since $|f_L(i) - f_{L + \xi \delta}(i)| \leq e_l^0(i) = e_r^0(i)$ for all $i \in [n]$ and $\xi \in [-1,\, 1]$ we see that any such profile $f_{L + \xi \delta}$ must eventually result in a consensus.


    If $L \leq 2$ the result follows immediately from Lemma \ref{thm:below2}.
%   Letting $d=\frac{1}{300}$, and so $n=1501$, we let $f$ be an equidistant profile with $n$ agents and diameter $L=5$. Noting that $d<\frac{1}{6}$ and that $\frac{1}{d}$ is even, we then use Corollary \ref{cor:step2} to bound the deviation $B_k^n(U^2f^{(2k)})-U^2f$, and denote the bounds obtained by $e_r^2$ and $e_l^2$. As this deviation is consistent, we can then use Corollary \ref{cor:devprop} to calculate bounds $e_r^5$ and $e_l^5$, and obtain that
%   \begin{equation*}
%         U^5f(n)+ e_r^5(n) - U^5f(1)-e_l^5(1) < 2.
%   \end{equation*}
%       [[explicita tal ska in här]]
% 
%   By Lemma \ref{lem:cont} this implies that the diameter of any sufficiently fine equidistant profile with initial diameter $L = 5$ must have shrunk below 2 after 5 updates, and the result now follows from Corollary \ref{cor:cons1}.
\end{proof}
\end{taggedblock}


















%  \begin{proof}
%  The idea is to show that the agents in $C_t$ will pull the agents in $A$ towards the centre until some time $t_1$ when the agent 1, called the \emph{extremist}, can see past the centre of the profile, at which point the diameter of the profile will be less than $2$ and thus eventually collapse by Theorem \ref{thm:below2}.
%  
%  To achieve this, we need to show a number of things:
%  \begin{enumerate}
%  \item We need to show that the sizes of the sets $C_t$ remain large enough to keep pulling at the extremist, the agent $1$. In fact, we will show that $C_t \subset C_{t+1}$ for all $t \geq t_0$.
%  \item We will show that the spans of opinions within the sets $A$ and $E$ are small for all $t \geq t_0$ such that no agent in $A$ has seen an agent in $E$ before $t$.
%  \item We need to show that the distance between the agents in $C_t$ and the extremist remains large enough for $t < t_1$. This will be used to ensure that the extremist in each step moves further than the sum of the spans of opinions within the sets $A$ and $E$, so that there is at most one time step when some agent in $A$ sees an agent in $E$ before $t_1$.
%  \end{enumerate}
%  [[Stryka listan??]]
%  
%  The proof will proceed by induction on $t$.
%  
%  Fix $t$ and assume for the rest of the proof that $C_t \supseteq C_{t-1} \supseteq ... \supseteq C_{t_0}$. Further, assume the sets $A_t$ and $E_t$ are mutually out of sight of one another, i.e. that $\mathcal{N}_{\max A} (U^t f) \cap E_t = \emptyset$.
%  
%  First, we will derive bounds $w_\mathcal{A}$ and $w_\mathcal{E}$ on the spans of opinions in the sets $A$ and $E$.
%  
%  Denote by $|\mathcal{A}_{t+1}|$ and $|\mathcal{E}_{t+1}|$ the spans of opinions in $A_{t+1}$ and $E_{t+1}$, respectively:
%  \begin{align}
%  |\mathcal{A}_{t+1}| &= U^{t+1} f(\max A_{t+1}) - U^{t+1} f(\min A_{t+1})\\
%  |\mathcal{E}_{t+1}| &= U^{t+1} f(\max E_{t+1}) - U^t f(\min E_{t+1}).
%  \end{align}
%  
%  Since, per definition, all agents in $A_t$ can see all agents in $C_t$, and we assume $E_t$ is out of sight, we know that $\mathcal{N}_{\max A}(U^t f) \setminus \mathcal{N}_{\min A}(U^t f) \subseteq D$. The case that pushes the two ends of $A$ to move as far apart as possible is that where the difference is all of $D$, and all where agents in the difference are placed at $U^tf(\max A) + 1$. We obtain the bound
%  \begin{align*}
%  |\mathcal{A}_{t+1}| & \leq \frac{|D_t|}{|A_t|+|B_t|+|C_t|+|D_t|} \leq \frac{2 |D_{t_0}|}{n - |E_{t_0}|} := w_\mathcal{A}.
%  \end{align*}
%  
%  Similarly we see that, by definition, $\mathcal{N}_{\max E_t} (U^t f) \setminus \mathcal{N}_{\min E_t} (U^t f) \subset B_t$. It is certainly impossible to separate the two ends more than if all of $B_t$ are visible to the agent $\min E_t$, while none are visible to the agent $\max E$, as the assumed symmetry will make the agents in the mirror image of $B_t$ pull $\max E_t$ in the other direction. After some manipulations, one finds
%  \begin{equation*}
%  |\mathcal{E}_{t+1}| \leq 2 \frac{|B_t|}{|B_t|+2|C_t|+2|D_t|+|E_t|} = \frac{2 |B_t|}{n - 2|A_t| - |B_t|} \leq \frac{2 |B_{t_0}|}{n - 2|A_{t_0}| - |B_{t_0}|} : = w_{\mathcal{E}}.
%  \end{equation*}
%  
%  [[Henceforth: $E_t = E$, $A_t = A$.]]
%  
%  We will now see that $C_{t+1} \supseteq C_t$ by checking for each of the sets $A_t$ and $E_t$ that they must remain in sight of any agent in $C_t$ after the update.
%  
%  Note that, as the updating operator is commutes with addition of constant functions, we may without loss of generality shift the profile without affecting the dynamics.
%  
%  For proving retained contact with the set $A$, we assume $\langle U^t f (i) \rangle_{i \in A} = 0$. The agents in $C_t$ can certainly not be moved further to the right than if all agents outside $C$ were placed in $c:=\frac{f(1)+f(n)}{2}$, the centre of the profile. As the diameter is decreasing, we get the bound
%  \begin{align*}
%  U^{t+1} f(\max C_t) &\leq \frac{2|B_t|+2|C_t|+2|D_t|+|E_t|}{|A_t|+2|B_t|+|C_t|+2|D_t|+|E_t|} \frac{L_t}{2}\\
%   & \leq \frac{(n-2|A_t|)/2}{(n-|A_t|)/2} \frac{L_t}{2}  \leq \frac{n-2|A|}{n-|A|} \frac{L_{t_0}}{2}
%  \end{align*}
%  Taking into account the spread of opinions in $A_{t+1}$, we get the bound
%  \begin{align*}
%  U^{t+1} f(\max C_t) - U^{t+1} f(1) & \leq \frac{n-2|A_t|}{n-|A_t|} \frac{L_{t_0}}{2} + |\mathcal{A}_{t+1}| \leq \frac{n-2|A_t|}{n-|A_t|} \frac{L_{t_0}}{2} + w_\mathcal{A} \\
%  & \leq \frac{n-2|A_{t_0}|}{n-|A_{t_0}|} \frac{L_{t_0}}{2} +  \frac{2 |D_{t_0}|}{n - |E|} \leq 1,
%  \end{align*}
%  where the last inequality holds by \eqref{eq:6tocons4}.
%  
%  We proceed similarly to prove retained contact with $E$. Assume now that the profile is symmetric around $0$, so that $f(1)+f(n) = 0$. An upper bound on the distance between the opinions in $C_t$ at time $t+1$ is obtained by placing all opinions outside $E_t$ in $\pm \frac{L_{t_0}}{2}$. This gives
%  \begin{align*}
%  U^{t+1} f(\frac{n+1}{2}) - U^{t+1} f(\min C_t) \leq \frac{(n-|E|)/2}{(n + |E|)/2} \frac{L_{t_0}}{2}.
%  \end{align*}
%  Taking the span of opinions into account, we find that
%  \begin{align*}
%  U^{t+1} f(\max E) - U^{t+1} f(\min C_t) \leq \frac{n-|E|}{n + |E|} \frac{L_{t_0}}{2} + \frac{2 |B_t|}{n - 2|A_t| - |B_t|} \leq 1
%  \end{align*}
%  where the last inequality holds by \eqref{eq:6tocons5}. This establishes $C_t \subseteq C_{t+1}$.
%  
%  We will now find a bound $s$ on the smallest possible step the extremist could move between times $t$ and $t+1$. A bound on this distance under the assumptions made can be obtained by placing the agents in $E$ at a distance just over $1$ away from the extremist, and all the rest of the agents on the lower half in the same cluster as the extremist. Updating, we see that
%  \begin{align*}
%  U^{t+1} f(\min C_t) - U^{t+1} f(1) \geq \frac{|E|}{(n-|E|)/2} := r.
%  \end{align*}
%  A lower bound on the step by the extremist can be obtained by considering a profile where $\mathcal{N}_1(U^t f) = A_t \cup B_t \cup C_t$, all opinions in $C_t$ are $r$ above the extremist and all agents in $B_t$ and $C_t$ are in a cluster with the extremist. The resulting movement would be
%  \begin{align*}
%  s := \frac{|C_t| r}{|A_t|+|B_t|+|C_t|} = \frac{|C_t|+|E_t|}{(|A_t|+|B_t|+|C_t|)(n-|A_t|)}.
%  \end{align*}
%  
%  We now observe that $s \geq w_\mathcal{A} + \frac{w_\mathcal{E}}{2}$, by the assumption in \eqref{eq:6tocons6}. For each $t \geq t_0$ this leaves two possibilities. The first is that no agent in $A$ can see any agent in $E$, in which case the structure of the profile is preserved until the next time step. If some agent in $A$ can instead see some agent in $E$ we know that by the next step the extremist will see past the centre of the profile, resulting in a consensus.
%  \end{proof}


















%  \begin{proof}[Proof of Theorem \ref{thm:6tocons}]
%    The proof will consist of four steps: First, we will show that the sets $C_{t}$ are increasing, in the sense that $C_{t} \subseteq C_{t+1}$ for all $t > t_00$.
%    
%    Second, we will show that the distance $U^tf(\min C_t) - U^tf(1)$ is bounded from below by some distance $r$ for each $t > t_0$ such that $\mathcal{N}_{\min E} (U^{t-1}f) \cap \mathcal{N}_{1} (U^{t-1}f) = \emptyset$. As the number $|C_t|$ of agents in $C_t$ is bounded from below, this will imply that the agents in $C_t$ will pull the extremist inwards by at least some amount $s$ at each time $t > t_0$.
%  
%    Third, we will show that we may then bound $|\mathcal{A}_t| < w_\mathcal{A}$ and $|\mathcal{E}_t| < w_\mathcal{E}$ for some constants $w_\mathcal{A}$ and $w_\mathcal{E}$ and every $t > t_0$ such that $\mathcal{N}_{\min E} (U^{t-1}f) \cap \mathcal{N}_{1} (U^{t-1}f) = \emptyset$.
%  
%    Fourth and finally, we will note that \eqref{eq:6tocons2} will imply $s \geq w_\mathcal{A} + \frac{w_\mathcal{E}}{2}$. We will see that this means that the extremists will keep moving inward until some time when they see past the centre of the profile, at which point Theorem \ref{thm:below2} completes the proof.
%    
%    For the proofs to come, we will employ a similar technique to some earlier proofs: We will construct profiles $g$ with $n$ agents, which satisfy the inequalities \eqref{eq:6tocons1} and \eqref{eq:6tocons2}, and which move certain agents as far as possible in some direction. We will thus show that the above mentioned assertions hold for our profiles $g$ and deduce that they must hold for any such profile. We use the same partitioning of the agents for the updates of the profile $g$ as for the profiles $U^{t_0}f$.
%  
%    By how the partition of the agents is constructed, we get upper bounds on the widths $|\mathcal{A}_t|$, $|\mathcal{C}_t|$ and $|\mathcal{E}_t|$.
%  
%    Construct a profile $g$ where $D = \mathcal{N}_{\max A}(g) \setminus\mathcal{N}_{\min A}(g)$ and where all agents in $D$ hold the opinion $g(\max A) + 1$. For this profile we have that
%    \begin{equation*}
%      Ug(\max A) - Ug(1) = \frac{|D_t|}{|A_t|+|B_t|+|C_t|+|D_t|} = \frac{|D_t|}{\left(n-|E_t|\right)/2}  = \frac{2 |D_t|}{n-|E_t|},
%    \end{equation*}
%    which implies
%    \begin{equation}
%      |\mathcal{A}_{t+1}| \leq \frac{2 |D_t|}{n-|E_t|}. \label{eq:6toconsa}
%    \end{equation}
%  
%    Loosening the requirement of symmetry, let $g$ be a profile with $n$ agents where $\mathcal{N}_{\max C_t}(g) \setminus \mathcal{N}_{\min C_t}(g) = n + 1 - \left( B_t \cup C_t \cup D_t \right)$, and where all agents in this set hold the opinion $g(\-ax C_t) + 1$. For this profile we have that
%    \begin{equation*}
%      Ug(\max C) - Ug(\min C) = \frac{|B_t|+|C_t|+|D_t|}{n-|A_t|} = \frac{n-2|A_t|-|E_t|}{2(n-|E_t|)},
%    \end{equation*}
%    which implies
%    \begin{equation}
%      |\mathcal{C}_{t+1}| \leq \frac{n-2|A_t|-|E_t|}{2(n-|E_t|)}.\label{eq:6toconsc}
%    \end{equation}
%    This bound must hold even if we reimpose the symmetry condition.
%  
%    Now, let $g$ be a symmetric profile with $n$ agents where $\mathcal{N}_{\min E_t} \setminus \mathcal{N}_{\max E_t} = B_t$, and where all agents in $B_t$ hold the opinion $g(\min E_t)-1$. For this profile, we have that
%    \begin{equation*}
%      Ug(\max E_t) - Ug(\min E_t) = \frac{|B_t|}{n - 2|A_t| - |B_t|},
%    \end{equation*}
%    which implies
%    \begin{equation}
%      |\mathcal{E}_t| \leq \frac{|B_t|}{n - 2|A_t| - |B_t|}. \label{eq:6toconse}
%    \end{equation}
%  
%    To prove that $C_{t} \subseteq C_{t+1}$ for all $t > t_0$, we will use induction. We will, without loss of generality, assume $f$ to be centred around $0$, in the sense that $f(1) + f(n) = 0$.
%  
%    We first consider the leftmost agent $\min C_{t_0}$ of $C_{t_0}$: Let $g$ be a symmetric profile with $n$ agents such that $\mathcal{N}_{\min C_t} = A_t \cup B_t \cup C_t \cup D_t \cup E_t$. To obtain a lower bound on $Uf(\min C_t)$, we construct $g$ so that all the agents in $A_t \cup B_t \cup C_t \cup D_t$ hold the opinion $-\frac{L_t}{2}$ and thus get
%    \begin{align}
%      Ug(\min C) &= \frac{-\frac{L_t}{2} \left(|A_t|+|B_t|+|C_t|+|D_t|\right)}{|A_t|+|B_t|+|C_t|+|D_t|+|E_t|} = \nonumber \\
%                 &= - \frac{n-|A_t|}{n+|A_t|} \frac{L_t}{2} 
%     \geq - \frac{n-|A_{t_0}|}{n+|A_{t_0}|} \frac{L_{t_0}}{2} \geq  -1 , \label{eq:6toconsminc}
%    \end{align}
%    where the last inequality follow from \eqref{eq:6tocons1}.
%  
%    We now note that \eqref{eq:6tocons3} implies that any agent in $C_{t+1}$ must be closer to the mean opinion of the agents in $A_t$, which we will denote $\bar{A_t}$, than to the mean of the agents outside $A_t$ and $n + 1 - A_t$, which, because of symmetry, is $0$. We thus have
%    \begin{align}
%      |U^{t_0}f(\max C_t) - U^{t_0}f(1)| & \leq |U^{t}f(\min C_t) - \bar{A_t}| + |\mathcal{A}_t| + |\mathcal{C}_t| \leq \nonumber\\
%      & \leq |U^{t}f(\min C_t)| + |\mathcal{A}_t| + |\mathcal{C}_t| \leq 1,
%    \end{align}
%    where the last inequality comes from substituting \eqref{eq:6toconsa}, \eqref{eq:6toconsc} and the second to last expression of \eqref{eq:6toconsminc}. The inequality then holds by \eqref{eq:6tocons1}.
%  
%    We have prooven that the sets $C_t$ are increasing. Looking at the definition, this implies that the sets $D_t$ are \emph{decreasing}, in the sense that $D_{t+1} \subset D_t$ for all $t \geq t_0$. The same holds for the sets $B_t$, and, by induction, we thus have $D_t \subset D_0$ and $B_t \subset B_0$ for all $t \geq t_0$, and so
%    \begin{equation}
%      |\mathcal{A}_t| \leq \frac{2 |D_0|}{n - |E_0|} , ~~~~~~~     |\mathcal{E}_t| \leq \frac{|B_0|}{n-2|A_0|-|B_0|} := w
%    \end{equation}
%    for all $t \geq t_0$. Defining the number $w$ is the third step in the plan laid out at the beginning of the proof.
%  
%    As for the fourth step, we will begin by bounding the distance between the extremist (which we call $1$) and the agent $\min C$. If the diameter of the profile would be smaller than $2$ we would be finished, so assume $L_t \geq 2$. By copying the steps leading up to \eqref{eq:6toconsminc}, we find that
%    \begin{equation}
%      U^tf(\min C_t) \geq - \frac{n-|A_0|}{n+|A_0|} \label{eq:6toconsminc2}
%    \end{equation}
%    for all $t \geq t_0$.
%    We may thus bound
%    \begin{equation}
%      U^tf(\min C_t) - U^tf(1) \geq
%      U^tf(\min C_t) + 1 \geq
%      1 - \frac{n-|A_0|}{n+|A_0|} \geq
%      \frac{2|A_0|}{n+|A_0|} :=
%      r \label{eq:6toconsr}
%    \end{equation}
%  
%    We may now, at last, bound the movement of the extremist as
%    \begin{equation}
%      U^{t+1}f(1) - U^tf(1) \geq \frac{|C_0| r}{|A_0|+|B_0|+|C_0|} = \frac{2|A_0||B_0|}{(n+|A_0|)(|A_0|+|B_0|+|C_0|)} := s
%    \end{equation}
%  
%    Finally, we conclude that \eqref{eq:6tocons2} implies that
%    \begin{equation}
%      s \geq w_\mathcal{A} + \frac{w_\mathcal{E}}{2} \label{eq:6toconsfinal}.
%    \end{equation}
%    We have this far showed that the extremists keep moving inward for as long as $\mathcal{N}_{\max A}(U^tf) \cap \mathcal{N}_{\min E}(U^tf) = \emptyset$, and \eqref{eq:6toconsfinal} assures us that if the two neighbourhoods ever overlap, the extremists will then move enough to ensure that $L_{t+1} \leq 2$. Theorem \ref{thm:below2} now completes the proof.
%  \end{proof}


% \begin{corollary}
%   Let $g_n$ be a profile with $n$ agents drawn independently and uniformly at random from an interval of length $L=6$. Then $\lim_{T \to \infty} U^Tg_n$ is a consensus a.a.s. as $n \to \infty$
% \end{corollary}


